Ranked Prioritization of Groups in Combinatorial Bandit Allocation

Preventing poaching through ranger patrols protects endangered wildlife, directly contributing to the UN Sustainable Development Goal 15 of life on land. Combinatorial bandits have been used to allocate limited patrol resources, but existing approaches overlook the fact that each location is home to multiple species in varying proportions, so a patrol benefits each species to differing degrees. When some species are more vulnerable, we ought to offer more protection to these animals; unfortunately, existing combinatorial bandit approaches do not offer a way to prioritize important species. To bridge this gap, (1) We propose a novel combinatorial bandit objective that trades off between reward maximization and also accounts for prioritization over species, which we call ranked prioritization. We show this objective can be expressed as a weighted linear sum of Lipschitz-continuous reward functions. (2) We provide RankedCUCB, an algorithm to select combinatorial actions that optimize our prioritization-based objective, and prove that it achieves asymptotic no-regret. (3) We demonstrate empirically that RankedCUCB leads to up to 38% improvement in outcomes for endangered species using real-world wildlife conservation data. Along with adapting to other challenges such as preventing illegal logging and overfishing, our no-regret algorithm addresses the general combinatorial bandit problem with a weighted linear objective.

==> figures/pareto_frontier.tex <==
\begin{tikzpicture}
\pgfplotsset{
  %scale only axis,
  width=.6\linewidth,
  height=.6\linewidth,
  xtick pos=left,
  ytick pos=left,
  tick label style={font=\scriptsize},
%   label style={font=\scriptsize},
%   ymajorgrids=true,
}


\pgfplotstableread[col sep=comma]{data/pareto_frontier_wildlife_N25_B5_G4.csv}\wildlifeparetodata;
\pgfplotstableread[col sep=comma]{data/pareto_frontier_covid_N41_B10_G3.csv}\covidparetodata;
\pgfplotstableread[col sep=comma]{data/pareto_frontier_family_van_N40_B10_G5.csv}\familyvanparetodata;

\begin{axis}[%
at={(0, 0)},
title={Wildlife Park},
xlabel={\small{Reward}},
ylabel={\small{Prioritization}},
every axis plot/.append style=only marks,
% every axis plot/.append style=scatter,
%   xlabel near ticks,
   ylabel near ticks,
  legend style={
    align=left,
    at={(2.4, 1.7)},
    legend columns=3,
    font=\small, 
    draw=none,
    fill=none,
    /tikz/every even column/.append style={column sep=0.15cm}},
]
	
\addplot [violet, mark=diamond*,
mark size=3pt, mark options={fill=violet},
    nodes near coords, % Place nodes near each coordinate
    point meta=explicit symbolic, % The meta data used in the nodes is not explicitly provided and not numeric
    every node near coord/.style={color=black, font=\scriptsize, anchor=south west}
] table [x=opt_reward, y=opt_fairness, meta index=1] {\wildlifeparetodata}; \addlegendentry{Optimal}
	
\addplot [mark=*, orange, mark options={fill=orange},
mark size=2pt,
    nodes near coords, % Place nodes near each coordinate
    point meta=explicit symbolic, % The meta data used in the nodes is not explicitly provided and not numeric
    every node near coord/.style={color=black, font=\scriptsize, anchor=south west}
] table [x=fair_reward, y=fair_fairness, meta index=2] {\wildlifeparetodata}; \addlegendentry{RankedCUCB}

\addplot [green!40!gray, mark=square*, mark options={fill=green!40!gray},
mark size=2pt,
    % nodes near coords, % Place nodes near each coordinate
    % point meta=explicit symbolic, % The meta data used in the nodes is not explicitly provided and not numeric
    % every node near coord/.style={color=black, font=\scriptsize, anchor=north west}
] table [x=lizard_reward, y=lizard_fairness, meta index=1] {\wildlifeparetodata}; \addlegendentry{LIZARD}
\end{axis}



\begin{axis}[%
at={(.45\linewidth, 0\linewidth)},
title={Synthetic},
xlabel={\small{Reward}},
%ylabel={Fairness},
every axis plot/.append style=only marks,
% every axis plot/.append style=scatter,
%   xlabel near ticks,
%   ylabel near ticks,
]


\addplot [violet, mark=diamond*,
mark size=3pt, mark options={fill=violet},
    nodes near coords, % Place nodes near each coordinate
    point meta=explicit symbolic, % The meta data used in the nodes is not explicitly provided and not numeric
    every node near coord/.style={color=black, font=\scriptsize, anchor=south west}
] table [x=opt_reward, y=opt_fairness, meta index=1] {\familyvanparetodata}; %\addlegendentry{Optimal}
	
\addplot [mark=*, orange, mark options={fill=orange},
mark size=2pt,
    nodes near coords, % Place nodes near each coordinate
    point meta=explicit symbolic, % The meta data used in the nodes is not explicitly provided and not numeric
    every node near coord/.style={color=black, font=\scriptsize, anchor=south west}
] table [x=fair_reward, y=fair_fairness, meta index=2] {\familyvanparetodata}; %\addlegendentry{FairUCB}

\addplot [green!40!gray, mark=square*, mark options={fill=green!40!gray},
mark size=2pt,
    % nodes near coords, % Place nodes near each coordinate
    % point meta=explicit symbolic, % The meta data used in the nodes is not explicitly provided and not numeric
    % every node near coord/.style={color=black, font=\scriptsize, anchor=north west}
] table [x=lizard_reward, y=lizard_fairness, meta index=1] {\familyvanparetodata}; %\addlegendentry{LIZARD}
\end{axis}

\end{tikzpicture}
